Human or LLM? A Comparative Study on Accessible Code Generation Capability

Web accessibility is essential for inclusive digital experiences, yet the accessibility of LLM-generated code remains underexplored. This paper presents an empirical study comparing the accessibility of web code generated by GPT-4o and Qwen2.5-Coder-32B-Instruct-AWQ against human-written code. Results show that LLMs often produce more accessible code, especially for basic features like color contrast and alternative text, but struggle with complex issues such as ARIA attributes. We also assess advanced prompting strategies (Zero-Shot, Few-Shot, Self-Criticism), finding they offer some gains but are limited. To address these gaps, we introduce FeedA11y, a feedback-driven ReAct-based approach that significantly outperforms other methods in improving accessibility. Our work highlights the promise of LLMs for accessible code generation and emphasizes the need for feedback-based techniques to address persistent challenges.

==> tables/achecker_results_qwen.tex <==
% \begin{table*}
% \centering
% \caption{Accessibility Evaluation for  Qwen2.5-Coder-32B-Instruct-AWQ (AChecker)}
% \label{tab:achecker_results_qwen}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|l|l|l|l|l} 
% \hline
% \multicolumn{1}{c|}{\textbf{Project}}  & \textbf{Human} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Naive Code}\\\textbf{Generation}\end{tabular}} & \multicolumn{1}{c|}{\textbf{Zero-Shot}} & \multicolumn{1}{c|}{\textbf{Few-Shot}} & \multicolumn{1}{c|}{\textbf{Self-Criticism}} & \multicolumn{1}{c}{\textbf{FeedA11y}}  \\ 
% \hline
% \textbf{vuejs/docs}                    & 0.4881         & 0.4959                                                                                                & 0.4959                                  & 0.4768                                 & 0.4527                                       & 0.4890                                 \\ 
% \hline
% \textbf{django/djangoproject.com}      & 0.8937         & 0.8399                                                                                                & 0.8399                                  & 0.6705                                 & 0.8399                                       & 0.6512                                 \\ 
% \hline
% \textbf{twbs/bootstrap}                & 0.1079         & 0.3230                                                                                                & 0.5907                                  & 0.6740                                 & 0.5902                                       & 0.2705                                 \\ 
% \hline
% \textbf{nodejs/nodejs.org}             & 0.5618         & 0.5259                                                                                                & 0.5390                                  & 0.4755                                 & 0.5280                                       & 0.4627                                 \\ 
% \hline
% \textbf{expressjs/expressjs.com}       & 0.3675         & 0.2193                                                                                                & 0.2230                                  & 0.4340                                 & 0.2859                                       & 0.2212                                 \\ 
% \hline
% \textbf{flutter/website}               & 0.3907         & 0.1957                                                                                                & 0.3138                                  & 0.6797                                 & 0.5468                                       & 0.1588                                 \\ 
% \hline
% \textbf{postgres/pgweb}                & 0.0546         & 0.0686                                                                                                & 0.0446                                  & 0.0759                                 & 0.1400                                       & 0.0666                                 \\ 
% \hline
% \textbf{foundation/foundation-sites}   & 0.8230         & 0.3850                                                                                                & 0.3194                                  & 0.5089                                 & 0.3756                                       & 0.3456                                 \\ 
% \hline
% \textbf{dart-lang/site-www}            & 0.3095         & 0.2535                                                                                                & 0.2154                                  & 0.2857                                 & 0.3446                                       & 0.1642                                 \\ 
% \hline
% \textbf{facebook/react-native-website} & 0.2545         & 0.1686                                                                                                & 0.1380                                  & 0.1634                                 & 0.1232                                       & 0.1683                                 \\ 
% \hline
% \textbf{AVG}                           & 0.4251         & 0.3475                                                                                                & 0.3720                                  & 0.4444                                 & 0.4227                                       & \textbf{0.2998}                        \\
% \hline
% \end{tabular}%
% }
% \end{table*}



% \begin{table}
% \centering
% \caption{Accessibility Evaluation for Qwen2.5-Coder-32B-Instruct-AWQ (AChecker)}
% \label{tab:achecker_results_qwen}
% \small
% \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l|c|c|c|c|c|c@{}}
% \hline
% \textbf{Project} & \textbf{H} & \textbf{N} & \textbf{Z} & \textbf{F} & \textbf{S} & \textbf{FA} \\ 
% \hline
% vuejs/docs & 0.49 & 0.50 & 0.50 & 0.48 & 0.45 & 0.49 \\ 
% django/djangoproject.com & 0.89 & 0.84 & 0.84 & 0.67 & 0.84 & 0.65 \\ 
% twbs/bootstrap & 0.11 & 0.32 & 0.59 & 0.67 & 0.59 & 0.27 \\ 
% nodejs/nodejs.org & 0.56 & 0.53 & 0.54 & 0.48 & 0.53 & 0.46 \\ 
% expressjs/expressjs.com & 0.37 & 0.22 & 0.22 & 0.43 & 0.29 & 0.22 \\ 
% flutter/website & 0.39 & 0.20 & 0.31 & 0.68 & 0.55 & 0.16 \\ 
% postgres/pgweb & 0.05 & 0.07 & 0.04 & 0.08 & 0.14 & 0.07 \\ 
% foundation/foundation-sites & 0.82 & 0.39 & 0.32 & 0.51 & 0.38 & 0.35 \\ 
% dart-lang/site-www & 0.31 & 0.25 & 0.22 & 0.29 & 0.34 & 0.16 \\ 
% facebook/react-native-website & 0.25 & 0.17 & 0.14 & 0.16 & 0.12 & 0.17 \\ 
% \hline
% \textbf{AVG} & 0.43 & 0.35 & 0.37 & 0.44 & 0.42 & \textbf{0.30} \\
% \hline
% \end{tabular*}

% \footnotesize H:Human, N:Naive, Z:Zero-Shot, F:Few-Shot, S:Self-Criticism, FA:FeedA11y
% \end{table}




% \begin{table*}
% \centering
% \caption{Accessibility Evaluation (AChecker) for GPT-4o and Qwen2.5-Coder}
% \label{tab:achecker_results_combined}
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l|c|cc|cc|cc|cc|cc@{}}
% \hline
% \multirow{2}{*}{\textbf{Project}} & \multirow{2}{*}{\textbf{H}} & \multicolumn{2}{c|}{\textbf{Naive}} & \multicolumn{2}{c|}{\textbf{Zero-Shot}} & \multicolumn{2}{c|}{\textbf{Few-Shot}} & \multicolumn{2}{c|}{\textbf{Self-Criticism}} & \multicolumn{2}{c}{\textbf{FeedA11y}} \\
% \cline{3-12}
%  & & \textbf{G} & \textbf{Q} & \textbf{G} & \textbf{Q} & \textbf{G} & \textbf{Q} & \textbf{G} & \textbf{Q} & \textbf{G} & \textbf{Q} \\
% \hline
% \textbf{vuejs/docs} & 0.488 & 0.475 & 0.496 & 0.500 & 0.496 & 0.488 & 0.477 & 0.475 & 0.453 & 0.475 & 0.489 \\
% \textbf{django/djangoproject.com} & 0.894 & 0.771 & 0.840 & 0.871 & 0.840 & 0.719 & 0.671 & 0.774 & 0.840 & 0.399 & 0.651 \\
% \textbf{twbs/bootstrap} & 0.108 & 0.153 & 0.323 & 0.128 & 0.591 & 0.355 & 0.674 & 0.318 & 0.590 & 0.185 & 0.271 \\
% \textbf{nodejs/nodejs.org} & 0.562 & 0.574 & 0.526 & 0.580 & 0.539 & 0.511 & 0.476 & 0.169 & 0.528 & 0.500 & 0.463 \\
% \textbf{expressjs/expressjs.com} & 0.368 & 0.293 & 0.219 & 0.293 & 0.223 & 0.315 & 0.434 & 0.302 & 0.286 & 0.205 & 0.221 \\
% \textbf{flutter/website} & 0.391 & 0.170 & 0.196 & 0.630 & 0.314 & 0.598 & 0.680 & 0.219 & 0.547 & 0.152 & 0.159 \\
% \textbf{postgres/pgweb} & 0.055 & 0.069 & 0.069 & 0.065 & 0.045 & 0.271 & 0.076 & 0.749 & 0.140 & 0.030 & 0.067 \\
% \textbf{foundation/foundation-sites} & 0.823 & 0.394 & 0.385 & 0.432 & 0.319 & 0.412 & 0.509 & 0.391 & 0.376 & 0.400 & 0.346 \\
% \textbf{dart-lang/site-www} & 0.310 & 0.338 & 0.254 & 0.234 & 0.215 & 0.654 & 0.286 & 0.172 & 0.345 & 0.343 & 0.164 \\
% \textbf{facebook/react-native-website} & 0.255 & 0.229 & 0.169 & 0.126 & 0.138 & 0.169 & 0.163 & 0.238 & 0.123 & 0.228 & 0.168 \\
% \hline
% \textbf{AVG} & 0.425 & 0.347 & 0.348 & 0.386 & 0.372 & 0.449 & 0.444 & 0.381 & 0.423 & \textbf{0.292} & \textbf{0.300} \\
% \hline
% \end{tabular*}

% \footnotesize \textbf{H}: Human, \textbf{G}: GPT-4o, \textbf{Q}: Qwen2.5-Coder, \textbf{Naive}: Naive Generation
% \end{table*}

==> tables/files.tex <==
\begin{table}
\centering
\caption{Number of Files}
\label{tab:number_of_files}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l} 
\hline
\textbf{Website Name}                  & \textbf{UI related files} & \textbf{Final size} & \textbf{Sampled size}  \\ 
\hline
\textbf{vuejs/docs}                    & 86                        & 82                  & 39                     \\ 
\hline
\textbf{django/djangoproject.com}      & 87                        & 54                  & 44                     \\ 
\hline
\textbf{twbs/bootstrap}                & 330                       & 217                 & 58                     \\ 
\hline
\textbf{nodejs/nodejs.org}             & 103                       & 45                  & 43                     \\ 
\hline
\textbf{expressjs/expressjs.com}       & 481                       & 441                 & 60                     \\ 
\hline
\textbf{flutter/website}               & 378                       & 352                 & 58                     \\ 
\hline
\textbf{postgres/pgweb}                & 71                        & 67                  & 36                     \\ 
\hline
\textbf{foundation/foundation-sites}   & 100                       & 48                  & 43                     \\ 
\hline
\textbf{dart-lang/site-www}            & 387                       & 370                 & 59                     \\ 
\hline
\textbf{facebook/react-native-website} & 59                        & 40                  & 33                     \\ 
\hline
\textbf{Total}                         & 2,792                     & 1,728               & 668                    \\
\hline
\end{tabular}%
}
\end{table}

==> tables/percentage.tex <==
\label{tab:percentage_achecker}


==> tables/projects.tex <==
\begin{table}
\centering
\caption{Selected Web Projects}
\label{tab:projects}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l|l} 
\hline
\textbf{Project}                       & \textbf{Commits} & \textbf{GitHub Stars} & \textbf{GitHub Contributors}  \\ 
\hline
\textbf{vuejs/docs}                    & 2,375            & 3k                    & 619                           \\ 
\hline
\textbf{django/djangoproject.com}      & 2,885            & 1.9k                  & 171                           \\ 
\hline
\textbf{twbs/bootstrap}                & 22,936           & 172k                  & 1,392                         \\ 
\hline
\textbf{nodejs/nodejs.org}             & 6,106            & 6.4k                  & 838                           \\ 
\hline
\textbf{expressjs/expressjs.com}       & 2,667            & 5.3k                  & 540                           \\ 
\hline
\textbf{flutter/website}               & 7,385            & 2.9k                  & 1,093                         \\ 
\hline
\textbf{postgres/pgweb}                & 2,356            & 77                    & 28                            \\ 
\hline
\textbf{foundation/foundation-sites}   & 17,309           & 29.7k                 & 1,039                         \\ 
\hline
\textbf{dart-lang/site-www}            & 4,158            & 979                   & 391                           \\ 
\hline
\textbf{facebook/react-native-website} & 3,691            & 2k                    & 1,304                         \\
\hline
\end{tabular}%
}
\end{table}

==> tables/qualweb_results.tex <==
\begin{table}
\centering
\caption{Accessibility Evaluation (QualWeb) for GPT-4o and Qwen2.5-Coder}
\label{tab:achecker_results_merged}
\small
\begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}}l|c|c|c|c|c|c@{}}
\hline
\textbf{Project} & \textbf{H} & \textbf{N} & \textbf{Z} & \textbf{F} & \textbf{S} & \textbf{FA} \\ 
\hline
vuejs/docs & 0.1655 / 0.1655 & 0.1116 / 0.1386 & 0.1520 / 0.1632 & 0.1735 / 0.1563 & 0.2508 / 0.1414 & 0.1632 / 0.1632 \\ 
django/djangoproject.com & 0.0213 / 0.0213 & 0.0284 / 0.0308 & 0.0239 / 0.0398 & 0.0546 / 0.0438 & 0.0343 / 0.0536 & 0.0249 / 0.0420 \\ 
twbs/bootstrap & 0.0611 / 0.0611 & 0.0701 / 0.0620 & 0.0696 / 0.0685 & 0.0816 / 0.0769 & 0.0815 / 0.0687 & 0.0820 / 0.0654 \\ 
nodejs/nodejs.org & 0.0209 / 0.0209 & 0.0184 / 0.0248 & 0.0410 / 0.0131 & 0.0258 / 0.0225 & 0.0220 / 0.0924 & 0.0246 / 0.0187 \\ 
expressjs/expressjs.com & 0.1444 / 0.1444 & 0.1147 / 0.1716 & 0.1393 / 0.1493 & 0.1423 / 0.1360 & 0.1104 / 0.2102 & 0.1690 / 0.1690 \\ 
flutter/website & 0.1789 / 0.1789 & 0.0283 / 0.0265 & 0.0387 / 0.0317 & 0.0277 / 0.0359 & 0.0279 / 0.0291 & 0.0312 / 0.0307 \\ 
postgres/pgweb & 0.0566 / 0.0566 & 0.0880 / 0.0912 & 0.0711 / 0.0840 & 0.0604 / 0.0564 & 0.0725 / 0.0910 & 0.0436 / 0.0665 \\ 
foundation/foundation-sites & 0.2658 / 0.2658 & 0.2611 / 0.2351 & 0.2630 / 0.2539 & 0.2445 / 0.2634 & 0.2487 / 0.2373 & 0.2501 / 0.1924 \\ 
dart-lang/site-www & 0.2103 / 0.2103 & 0.2360 / 0.2271 & 0.2182 / 0.2563 & 0.2627 / 0.2090 & 0.2087 / 0.2045 & 0.2227 / 0.2227 \\ 
facebook/react-native-website & 0.1211 / 0.1211 & 0.0974 / 0.1211 & 0.0981 / 0.1529 & 0.1018 / 0.1078 & 0.0667 / 0.0866 & 0.1041 / 0.1011 \\ 
\hline
\textbf{AVG} & 0.1246 / 0.1246 & 0.1054 / 0.1129 & 0.1115 / 0.1213 & 0.1175 / 0.1108 & 0.1124 / 0.1215 & \textbf{0.1115 / 0.1072} \\
\hline
\end{tabular*}

\footnotesize H:Human, N:Naive, Z:Zero-Shot, F:Few-Shot, S:Self-Criticism, FA:FeedA11y \\
\footnotesize Values are formatted as GPT-4o / Qwen2.5-Coder
\end{table}

